EverLight: Indoor-Outdoor Editable HDR Lighting Estimation

Because of the diversity in lighting environments, existing illumination estimation techniques have been designed explicitly on indoor or outdoor environments. Methods have focused specifically on capturing accurate energy (e.g., through parametric lighting models), which emphasizes shading and strong cast shadows; or producing plausible texture (e.g., with GANs), which prioritizes plausible reflections. Approaches which provide editable lighting capabilities have been proposed, but these tend to be with simplified lighting models, offering limited realism. In this work, we propose to bridge the gap between these recent trends in the literature, and propose a method which combines a parametric light model with 360{\deg} panoramas, ready to use as HDRI in rendering engines. We leverage recent advances in GAN-based LDR panorama extrapolation from a regular image, which we extend to HDR using parametric spherical gaussians. To achieve this, we introduce a novel lighting co-modulation method that injects lighting-related features throughout the generator, tightly coupling the original or edited scene illumination within the panorama generation process. In our representation, users can easily edit light direction, intensity, number, etc. to impact shading while providing rich, complex reflections while seamlessly blending with the edits. Furthermore, our method encompasses indoor and outdoor environments, demonstrating state-of-the-art results even when compared to domain-specific methods.

==> notes.tex <==
\section{Notes}
\listoftodos

Papers are limited to eight pages, including figures and tables, in the ICCV style. Additional pages containing only cited references are allowed. Appendices may not be a part of the additional pages. Appendices are counted towards the eight-page limit or should be moved to the supplementary document. Please refer to the following files for detailed formatting instructions:

\begin{enumerate}
    \item Appendix
    \item Supplemental Material
    \begin{enumerate}
        \item loss curves
    \end{enumerate}
\end{enumerate}
